Insecticide treated bed net use and elimination of malaria in Sub-Saharan African countries: Assessing the Global Technical Strategy (GTS) using an evolutionary game approach

The WHO 2021 malaria report revealed that its Global Technical Strategy (GTS) 2020 milestones for morbidity and mortality, based on the 2015 baseline, have not been achieved globally -- the world is off-track by 42% and, can be extended up to 91% in 2030. Most of the Sub-Saharan African (SSA) countries failed to achieve GTS 2020 -- only 4 out of 40 highest burden countries met the goals. By fitting evolutionary game modeling to the malaria case and Insecticide-Treated Nets (ITN) usages data, we identify factors contributing to the GTS 2020 failures of 38 SSA countries. We use optimized projection of our model to evaluate further the potential achievement of GTS 2025 and 2030 objectives and discuss strategies for attaining goals in situations where these milestones seem unattainable. Our findings categorize all 38 countries based on the possibility to achieve their future milestone, either through increased campaigns, or by economic assistance, or through enhancing the efficacy of ITNs at minimal expense.

==> latexmkrc <==
$sub_doc_output = 'output-subdoc';

@sub_doc_options = ();

push @sub_doc_options, '-pdf'; # Use pdflatex for compilation of external documents.
# Replace '-pdf' by '-pdfdvi', 'pdfxe', or 'pdflua' if needed.

push @file_not_found, '^No file\\s*(.+)\s*$';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if ( $root_filename ne $_[0] )  {
        my ($base_name, $path) = fileparse( $_[0] );
        pushd $path;
        my $return = system "latexmk",
                            @sub_doc_options,
                            "-aux-directory=$sub_doc_output",
                            "-output-directory=$sub_doc_output",
                            $base_name;
        if ( ($sub_doc_output ne ' ') && ($sub_doc_output ne '.') ) {

             rdb_add_generated( "$sub_doc_output/$base_name.aux" );
             copy "$sub_doc_output/$base_name.aux", ".";
        }
        popd;
        return $return;
   }
}
